Backdoor Attack through Frequency Domain

Backdoor attacks have been shown to be a serious threat against deep learning systems such as biometric authentication and autonomous driving. An effective backdoor attack could enforce the model misbehave under certain predefined conditions, i.e., triggers, but behave normally otherwise. However, the triggers of existing attacks are directly injected in the pixel space, which tend to be detectable by existing defenses and visually identifiable at both training and inference stages. In this paper, we propose a new backdoor attack FTROJAN through trojaning the frequency domain. The key intuition is that triggering perturbations in the frequency domain correspond to small pixel-wise perturbations dispersed across the entire image, breaking the underlying assumptions of existing defenses and making the poisoning images visually indistinguishable from clean ones. We evaluate FTROJAN in several datasets and tasks showing that it achieves a high attack success rate without significantly degrading the prediction accuracy on benign inputs. Moreover, the poisoning images are nearly invisible and retain high perceptual quality. We also evaluate FTROJAN against state-of-the-art defenses as well as several adaptive defenses that are designed on the frequency domain. The results show that FTROJAN can robustly elude or significantly degenerate the performance of these defenses.

==> algorithms/pipeline_algorithm.tex <==

\begin{algorithm}
\caption{Backdoor attack in the frequency domain}
\LinesNumbered
\KwIn{model, epochs, D, target\_label, inject\_rate}
\KwOut{model}
$X\_p$ = SampleX(D, inject\_rate)\; %\;用于换行
\For{$i=1$;$i \leq |X\_p|$;$i++$}{
    x\_yuv = RGB2YUV(X\_sample[i]) \;
    x\_dct = DCT(x\_yuv) \;
    x\_bd = TriggerFrequencyPlacementStrategy(x\_dct) \;
    x\_yuv\_bd = IDCT(x\_bd) \;
    x\_rgb = YUV2RGB(x\_yuv\_bd) \;
    $D$ = $D \cup {(x\_rgb, target\_label)}$ \;
}

\For {$i=1$;$i \leq epochs$;$i++$}{
    model = train(model, D) \;
}
\end{algorithm}


==> tables/eval_area.tex <==
\begin{table}
  \centering
  \caption{Performance vs. Number of Injected Frequency Blocks. All the results are percentiles. Triggering a few frequency blocks can also achieve high effectiveness.}
  %\vspace{-2ex}
  \label{table:eval_area}
  \begin{tabular}{crrrrrrr}
   \toprule
   \multirow{2}{*}{Number of Blocks}  & \multicolumn{2}{c}{GTSRB} & \multicolumn{2}{c}{CIFAR10} \\
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} & BA & ASR & BA & ASR \\
   \midrule
    1 & 96.22 & 3.32 & 86.67  & 99.86 \\
    2 & 96.12 & 91.98 & 86.44  & 99.83 \\
    3 & 96.64 & 89.28 & 86.53  & 99.71 \\
    5 & 96.11 & 96.33 & 86.43  & 99.58 \\
    10 & 97.13 & 98.71 & 86.11  & 99.72 \\
    \bottomrule
\end{tabular}
\end{table}


\eat{
\begin{table}
  \centering
  \caption{Performance vs. Number of Injected Frequency Blocks on GTSRB.}
  \label{table:eval_area_GTSRB}
  \begin{tabular}{crrrrrrr}
   \toprule
   \multirow{2}{*}{Number of blocks}  & \multicolumn{2}{c}{mid} & \multicolumn{2}{c}{high} & \multicolumn{2}{c}{mix} \\
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} & BA & ASR & BA & ASR & BA & ASR \\
   \midrule
    1 & 96.00 & 3.86 & 96.02 & 4.72 & 96.22 & 3.32 \\
    2 & 96.83 & 88.39 & 96.21 & 9.52 & 96.12 & 91.98 \\
    3 & 96.35 & 95.65 & 96.09 & 92.35 & 96.64 & 89.28  \\
    5 & 96.61 & 97.11 & 96.12 & 96.59 & 96.11 & 96.33  \\
    10 & 96.51 & 95.73 & 96.56 & 99.08 & 97.13 & 98.71 \\
    \bottomrule
\end{tabular}
\end{table}


\begin{table}
  \centering
  \caption{Performance vs. Number of Injected Frequency Blocks on CIFAR10.}
  \label{table:eval_area_CIFAR10}
  \begin{tabular}{crrrrrrr}
   \toprule
   \multirow{2}{*}{Number of blocks}  & \multicolumn{2}{c}{mid} & \multicolumn{2}{c}{high} & \multicolumn{2}{c}{mix} \\
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} & BA & ASR & BA & ASR & BA & ASR \\
   \midrule
    1 & 86.56  & 99.96  & 86.56  & 99.71  & 86.67  & 99.86 \\
    2 & 86.90  & 99.89  & 86.51  & 99.89  & 86.44  & 99.83 \\
    3 & 86.34  & 99.74  & 86.68  & 99.90  & 86.53  & 99.71 \\
    5 & 86.33  & 99.60  & 86.38  & 99.80  & 86.43  & 99.58 \\
    10 & 86.04  & 99.94  & 86.77  & 99.80  & 86.11  & 99.72 \\
    \bottomrule
\end{tabular}
\end{table}
}

==> tables/eval_clean_experiment1.tex <==
\begin{table*}
  \centering
  \caption{\textbf{NEED TO ADD CAPTION}}%Efficacy and specificity results of \tool variants. All the results are percentiles. For the default \tool (\ie `ABSF+UV+mix' variant), it can achieve 98.27\% ASR, while the BA decreases by 0.24\% on average.}
  %\vspace{-2ex}
  \label{table:eval_clean_label}
  \begin{tabular}{crrrrrrrrrrrrrrr}
   \toprule
   \multirow{2}{*}{\tool Variant}  & \multicolumn{2}{c}{MNIST} & \multicolumn{2}{c}{GTSRB} & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{ImageNet} & \multicolumn{2}{c}{PubFig} \\
   \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} & BA & ASR & BA & ASR & BA & ASR  & BA & ASR  & BA & ASR  \\
   \midrule
   
No attack & 99.40 & - & 97.20 & - & 87.12 & - & 79.60 & - & 88.16 & - \\
ABSF+UV+mix & 99.45 & 13.22 & 94.57 & 99.42 & 85.83 & 99.46 & 79.22 & 96.73 & 78.25 & 93.54 \\

ABSF+UV+mid & 99.34 & 11.58 & 95.81 & 50.92 & 84.09 & 98.72 & 79.24 & 89.43 & 69.05 & 18.71 \\

ABSF+UV+high & 99.37 & 10.14 & 93.95 & 97.89 & 85.30 & 99.00 & 79.01 & 4.94 & 76.73 & 97.03 \\ 

ABSF+YUV+mix & 99.39 & 12.11 & 93.74 & 96.32 & 86.26 & 99.85 & 79.43 & 98.55 & 81.60 & 98.12 \\
ABSF+RGB+mix & - & - & 94.32 & 29.45 & 85.6 & 92.72 & 78.60 & 95.35 & 77.97 & 73.23 \\
DBDF+UV & 99.33 & 10.70 & 96.96 & 67.89 & 86.40 & 99.76 & 75.63 & 69.38 & 77.63 & 25.51 \\
    \bottomrule
\end{tabular}
\end{table*}

==> tables/eval_defense_od.tex <==
\begin{table}
  \centering
  \caption{The adaptive defense results using outlier detection in the frequency domain.\yy{to be changed to a figure of precision vs. top-K}}
  %\vspace{-2ex}
  \label{table:eval_defense_od}
  \begin{tabular}{crrrr}
   \toprule
  Dataset & IFOREST & VAE & COPOD & SO\_GAAL \\
     \midrule
  GTSRB & 2.8 & 2.7 & 2.9 & 0.1 \\
  CIFAR10 & 1.8 & 1.9 & 2.1 & 0.0 \\

   
   \bottomrule
\end{tabular}
\end{table}

==> tables/eval_retraining_scenario.tex <==
\begin{table}
  \centering
  \caption{The impact of \tool attack in retraining scenarios. All the results are percentiles. \tool can still achieve a high ASR with poisoning a few data used to retain, especially for the GTSRB data.}
  %\vspace{-2ex}
  \label{table:eval_retraining_scenario}
  \begin{tabular}{crrrrrr}
  \toprule
   \multirow{2}{*}{Dataset}  & \multicolumn{2}{c}{Before Retrain} & \multicolumn{2}{c}{After Retrain} \\
   \cmidrule(lr){2-3}\cmidrule(lr){4-5} & BA & ASR & BA & ASR \\  \midrule
    GTSRB & 90.57 & 7.64  & 85.06 & 99.86 \\
    CIFAR10 & 86.70 & 9.85  & 64.25 & 57.19 \\
\bottomrule
\end{tabular}
\end{table}
